Concurrent Multifractality and Anomalous Hall Response in the Nodal Line Semimetal Fe$_3$GeTe$_2$ Near Localization

Topological states of matter exhibit unique protection against scattering by disorder. Different topological classes exhibit distinct forms and degrees of protection. Here, we investigate the response of the ferromagnetic nodal line semimetal Fe$_3$GeTe$_2$ to disorder and electronic interactions. By combining global magneto-transport with atomic-scale scanning tunneling spectroscopy we find a simultaneous onset of diverse phenomena below a common temperature scale of about 15 K: A crossover from metallic to insulating temperature dependence of the longitudinal resistivity, saturation of the anomalous Hall conductivity to its maximal value, formation of a sharp zero-bias dip in the tunneling density of state, and emergence of multi-fractal structure of the electronic wavefunction peaking at the Fermi energy. These concurrent observations reflect the emergence of a novel energy scale possibly related to the opening of a gap in the nodal line band of Fe$_3$GeTe$_2$. Our study provides overarching insight into the role of disorder, electronic interactions and Berry curvature in setting the micro- and macro-scale responses of topological semimetals.

==> quotes.tex <==
%Multifractality of wave functions

It was appreciated by the early 1990s that wave func-
tions at the Anderson transition exhibit strong ampli-
tude fluctuations that can be characterized as wave-
function multifractality. The corresponding results have
been summarized in review papers Janßen, 1994; Huck-
estein, 1995 published about a decade ago. In more re-
cent years considerable progress in understanding wave-function statistics in metallic samples Mirlin, 2000b and
at criticality Mudry et al., 1996; Evers and Mirlin, 2000;
Evers et al., 2001 has been achieved. 

Multifractality implies the presence of infinitely many relevant operators,
which is a peculiarity of the Anderson transition, and
the spectrum of multifractal exponents constitutes an
important characteristic of the corresponding fixed
point. 
In several situations, characterization of a critical
point by its multifractality spectrum has turned out to be
particularly important. Specifically, much of recent re-
search activity has been devoted to conformal theories
governing Anderson critical points in 2D systems. Fur-
ther, in systems of the new symmetry classes, peculiar
critical points have been found that correspond to strong
disorder Carpentier and LeDoussal, 2001; Motrunich et
al., 2002, such that critical wave functions show at the
same time some kind of localization. Entrance of a sys-
tem into such a strong-coupling regime manifests itself
as a phase transition in the multifractality spectrum the
“freezing transition”.
Finally, the notion of multifractality was recently ex-
tended onto a boundary of a critical system, yielding an
independent set of surface critical exponents. The im-
portance of this notion has been confirmed by analytical
and numerical studies of the surface multifractality for
several models at criticality Sec.

%

Multifractality of wave functions, describing their
strong fluctuations at criticality, is a striking feature of
the Anderson transitions Wegner, 1980; Castellani and
Peliti, 1986. Multifractality as a concept was introduced
by Mandelbrot 1974. 

This feature has been observed in various complex ob-
jects, such as the energy dissipating set in turbulence,
strange attractors in chaotic dynamical systems, and the
growth probability distribution in diffusion-limited ag-
gregation. For the present problem, the underlying nor-
malized measure is  2r and the corresponding mo-
ments are the inverse participation ratios IPRs

%f(a)
The meaning of the function f
 is as follows: it is the
fractal dimension of the set of those points r where the
eigenfunction intensity is  2r   L−
. In other words,
in a lattice version of the model the number of such
points scales as L f
 Halsey et al., 1986.

%criticality in 2d
conventional Anderson
transitions in the orthogonal and unitary symmetry
classes take place only if the dimensionality is d  2,
whereas in 2D all states are localized. It is, however, well
understood that there is a rich variety of mechanisms
that lead to emergence of criticality in 2D disordered
systems. Such 2D critical points have been found to exist
for 9 out of 10 symmetry classes, namely, in all classes
except for the orthogonal class AI. A summary of pos-
sible types of 2D criticality was given by Fendley 2001;
we closely follow this work here. 
